Equity and Privacy: More Than Just a Tradeoff

While the entire field of privacy preserving data analytics is focused on the privacy-utility tradeoff, recent work has shown that privacy preserving data publishing can introduce different levels of utility across different population groups. It is important to understand this new tradeoff between privacy and equity as privacy technology is being deployed in situations where the data products will be used for research and policy making. Will marginal populations see disproportionately less utility from privacy technology? If there is an inequity how can we address it?

==> Pastebin.tex <==
\section{Remedies}
While it might seem like privacy and equity are fundamentally at odds with each other as we have presented it we want to discuss here how that's not inherently the case and how there are cases where privacy and equity can coexist. The examples we've shown here demonstrate what happens when differentially private systems do not adjust for the noise being introduced. However, one of the benefits of differential privacy is that the noise distribution is often known in advance and mechanism being run on privacy protected data can adapt to this noise and it's affects on minority populations. It's also important to recognize and understand that privacy and it's tradeoffs do not exist in a vacuum but are a part of a society as a whole and that some methods of removing the minority disparity result in shifting the privacy-utility tradeoff to another dimension which still disproportionately affect minority groups. \am{I do not understand the points made in this paragraph ... Can you highlight what the key points you want to make in this section are?}

\am{Maybe an idea for this section is: 
\begin{itemize}
\item Intro section that says there are two problems: (a) the data released by privacy methods s noisy (and not true data), and (b) that noise introduced by privacy methods in combination with unbalanced population groups seem to be causing the equity problem. To combat the former, downstream methods should take into account the privacy protection methods used. Under differential privacy this is often easy to do since the noise distributions and their scales are known a priori. 
For the latter ... you talk a bit about oversampling and why you think this is a bad idea.
\item Discuss the allocation problem remedies (a summary of what you have for Pujol and Fioretto)
\item Discuss the ML problem: a short para summarizing the first two paras of conclusion. 
\end{itemize}
}

First, we want to address the simplest solution to some of the problems seen here. Primarily that of data collection. In the previous machine learning tasks we seen that small sub-populations tend to see increased utility loss for the same privacy protections. This result was the same if the sub-populations are reflective of actual minority groups or simply remnants of undersampling data. In this case the solution seems clear, simply collect more data about these minority groups in order to reduce their utility loss. We would argue that this is simply replacing one tradeoff with another, this time a more socieotechnical one. Where before, there was a tradeoff between utility and privacy there is now a tradeoff between surveillance and utility. By collecting additional data from minority groups you are imposing more surveillance on a population who is often already under increased surveillance (often without recourse). This method doesn't alleviate the burden placed on minorities but instead forces them to pay elsewhere.   \par

There are alternative approaches to reducing the disparity caused by privacy protections. The first method is adapting decision making processes to the added noise. 

Unlike other sources of noise the noise introduced by differentially private mechanisms and other privacy preserving techniques are often known ahead of time. In the case of differential privacy noise is usually sampled from either the Laplace Distribution or the Gaussian Distribution. Since these distributions are known ahead of time the decision tasks can be adapted in order to properly account for the noise. For example in the Pujol et al. paper \cite{PujolMKHMM20} the authors introduce a method for reducing the impact of privacy on the title one funding allocation. They suggest slightly inflating the overall budget and distributing the additional budget in a way to counteract the biases introduced by the differentially private mechanism. By doing this they can ensure that with high probability no school district is punished and receives a lower allocation of funds than in the non-private version of the same allocation task. This method leverages the known distribution of noise in order to ensure some definition of equity, in the same way various other allocation tasks could analyze and adapt to the presence of known noise in the data. This method also shifts the tradeoff between utility and privacy but instead of moving the burden onto the minority group it moves the burden onto the one allocating resources by requiring slightly more resources than the initial allocation. Building on this case Fioretto et al. \cite{FairPrivFollowup} demonstrate that for class of allocation functions (those where the entries of their hessian are constant functions) the equity loss due to privacy can be bounded and that the problems introduced by Pujol et al. \cite{PujolMKHMM20} are not in this class. This suggests that the allocation functions themselves can be replaced by similar functions which behave more equitably in the face of noise.

\section{Conclusion}
As a new field of research not much is known directly about the interaction between privacy and equity. Most of what is known are from empirical studies that show cases in which privacy and equity are at odds. While this work is essential in exploring the relationship between privacy and equity in different settings it does not prove the existence of any fundamental relationship between privacy and equity. In order to understand this relationship it must be studied theoretically through provable mathematical theorems. Both the fields of privacy and equity have shown many theoretical results independently but not much known about their interactions. \par 
Though the theoretical work between privacy and equity is sparse the theoretical result that have emerged have created an equal amount of practical results. Cummings et al. \cite{FairPrivCombatibility} recently described the interactions between differential privacy and equal opportunity, a notion of equity that requires equal true positive classification rates across groups. They showed there there does not exist a classifier which achieves differential privacy, equalized odds and has accuracy higher than a constant classifier. Though this may seem like a stark negative result the understanding gained by this work has lead to equally positive results. Jagielski et al. \cite{DPFairLearning} have shown two algorithms which satisfy equalized odds and an approximate notion of differential privacy. Likewise, Tran et al.  \cite{DualApproach} develop a method of satisfying several group notions of equity and approximate differential privacy by using a Lagrangian dual approach. Both of these developments accept the impossibility result of Cummings et al. and adapt to it by using approximate differential privacy as opposed to pure differential privacy. \par 
\am{We may be running out of words at this point. So it might be useful to summarize these two paragraphs into a couple of sentences \& maybe even move it to the Remedies (?) section  -- 
\begin{itemize}
    \item We discussed case studies that empirically show the privacy-equity tradeoff.  Is there a fundamental theoretical relationship between the two? 
    \item There is emerging theoretical work in this space that suggests that this tradeoff is fundamental \cite{} for "pure"-differential privacy, but the negative results can be overcome in an "approximate" regime of differential privacy \cite{}. 
\end{itemize}
I made a pass on the last paragraph, which should be the conclusion.
}


